3DPFIX: Improving Remote Novices' 3D Printing Troubleshooting through Human-AI Collaboration

The widespread consumer-grade 3D printers and learning resources online enable novices to self-train in remote settings. While troubleshooting plays an essential part of 3D printing, the process remains challenging for many remote novices even with the help of well-developed online sources, such as online troubleshooting archives and online community help. We conducted a formative study with 76 active 3D printing users to learn how remote novices leverage online resources in troubleshooting and their challenges. We found that remote novices cannot fully utilize online resources. For example, the online archives statically provide general information, making it hard to search and relate their unique cases with existing descriptions. Online communities can potentially ease their struggles by providing more targeted suggestions, but a helper who can provide custom help is rather scarce, making it hard to obtain timely assistance. We propose 3DPFIX, an interactive 3D troubleshooting system powered by the pipeline to facilitate Human-AI Collaboration, designed to improve novices' 3D printing experiences and thus help them easily accumulate their domain knowledge. We built 3DPFIX that supports automated diagnosis and solution-seeking. 3DPFIX was built upon shared dialogues about failure cases from Q&A discourses accumulated in online communities. We leverage social annotations (i.e., comments) to build an annotated failure image dataset for AI classifiers and extract a solution pool. Our summative study revealed that using 3DPFIX helped participants spend significantly less effort in diagnosing failures and finding a more accurate solution than relying on their common practice. We also found that 3DPFIX users learn about 3D printing domain-specific knowledge. We discuss the implications of leveraging community-driven data in developing future Human-AI Collaboration designs.

==> sections/deprecated.tex <==

%\section{\system: A Pipeline to Build an Interactive System for Automatic Problem Diagnosis \& Solution-Recommendation Powered by \notion} \label{implementation}


\subsection{\system Overview} \label{system_overview}
\jk{also add the figure that describes a user walkthrough: uploading image, seeing the list of issues diagnosed, choose one to see solutions, etc.}
%\jk{it's weird that the system overview is here after all details about how the pipeline is built.}

\system is an interactive web application that provides automatic AI-diagnosis of 3D printing failure and recommends corresponding solutions based on a user-uploaded photo.
% Powered by AI
.
% and provides various suggestions extracted from existing discussions in the online community.
\system can identify and suggest relevant solutions for 5 common types of printing failure that present distinct visual features (as in Section~\ref{visual_features}): stringing, under-extrusion, layer shifting, warping, and blobs, as shown in Figure~\ref{}.
The automatic diagnosis of failure types is backed up by 5 binary classification models. 
% After a user upload an image,  to determine whether the input image contains each.

\jk{add the most representative image of 5 failure type what 3DFix can find}
\nk{do we still need another figure for representative images other than visual features figure? if so, what would be the representative images? images in simplify3d?}
%, due to multi-class property of failed 3D prints (\textit{i.e.}, a single 3D print can have visual characteristics of multiple failures ( Figure~\ref{figure:multiple_failure}).


\system contains three main features: (1) the system diagnoses failure types from user-uploaded photos and presents the grayscale saliency attention map that shows how the models make the prediction powered by a CNN model; (2) the system presents instructional materials to help users learn the diagnosed failure types with description and images; (3) The systems provides common \& tailored solution sets based on the diagnosed failure. We elaborate the features of \system in this section.


\subsubsection{Example User Workflow}
We describe an example user workflow of \system with a speculative user Teddy.
Teddy found that his printed object has a lot of gaps on the surface, which makes the outer wall very weak all over the model. %tried yyy which did not completely resolved the case.
% } 
He does not know what to call the problem, thus takes a photo of his failed print and uploads it on \system.
%If desired, they can upload mutliple photos at once. They can explore each image by clicking thumbnail images at the top.
He can get the diagnosed failure types along with the grayscale saliency maps that shows the highlighted area with the unique visual characteristics of the failure identified by the system. 
\system first shows the most likely failure types by default.
The only highly likely failure type \system diagnosed is under-extrusion, but he also wants to check all other possible failure types to make sure that AI made the right decision. 
He clicks the `Show All Failure Types' button, and check the sample images that inform common visual characteristics of each failure under the `What's this Problem?' tab to compare those to his model.
By looking at all possible options, Teddy is sure that his problem is under-extrusion, as his print has `spongy pattern' on the surface as shown in common visual characteristics of under-extrusion.
%but if needed, he can also decide which failure type to address %by checking AI's decision on all failure types that \system supports. 
Upon selecting under-extrusion type to explore, Teddy can learn about under-extrusion by looking at the description.%. and representative images that cover possible different appearance of the failure.
If Teddy thinks that he understood the details about under-extrusion enough, he can also check the common solutions which are likely to solve the most of cases. 
He tried all the common solution listed, but he finds out that the problem still remains unsolved. His case might be unique in that it cannot be solved by common solutions. 
If so, he can proceed to the specific solutions tab which covers most possible cases extracted from the online community discussion.
By going through the clue list that shows the possible situations or settings he might have, he read one clue there, `I heard a popping noise when it leaves a gap'. Then he remembers that he heard a weird noise when he printed that object. 
He clicks that clue, and \system shows one related solution card says that it might be an issue of a wet filament.
He did not know about the wet filament can cause this type of problem, so he read the linked web article by clicking a `View Detail' button on the solution card.
By reading the article, he learns that the wet filament can cause multiple problem such as under-extrusion and blobbing.
As he does not have any gadget to dry the filament, he finally solves the issue by replacing the filament with the new sealed one.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/3DPFIX_diagnosis.png}
    \caption{This is the top section of the interface where users can select the 3D printing images they uploaded for diagnosis (upper subsection) and the corresponding failure type predictions with saliency maps generated by our models (lower subsection). Images are clickable tabs where red-colored borders indicate active selections. The system also displays the likelihood of each failure type predictions (Highly Likely: 75\% - 100\%, Likely: 50\% - 75\%, Unlikely: 25\% - 50\%, and Highly Unlikely: 0\% - 25\%). Users can click a specific failure prediction to explore further about the solutions on the bottom section of the interface shown in Figure \ref{figure:system_description}, \ref{figure:system_solutions}, \ref{figure:system_hoverover}. Users can also use the toggle switch buttons to ``Show All Failure Types'' or ``Show AI's Best Guess'' which filters out the predictions below the "Highly Likely" level.}
    \Description{}
    \label{figure:system_diagnosis}
    %  \vspace{-2.0ex}
\end{figure*}

\subsubsection{User benefit 1: Automatic Failure Diagnosis.}
Once the users upload the photo (s), \system calculates the prediction probability of having failure types using all classification models step by step.
As the prediction per one image takes less than 10 seconds, \system can address \textit{immediacy} in comparison to the feedback from other users in online communities (\textit{Design Consideration 1. immediacy, 2. image-based diagnosis})
%3DPFIX displays the failure type with the probability of 75\% or above, which is the current threshold.
%For example, Figure~\ref{figure:ui_image_diagnosis} shows that the user-uploaded photo has only an under-extrusion problem, which showed 84.5\% probability, while the probabilities for other failure types are less than 75\%.
Although displaying a probability is a common approach in designing intelligent systems to increase explainability \cite{} \jk{missing citation to back up}, \system does not show prediction probabilities to the end-users.
This design decision intends not to confuse users in interpreting the numeric values \cite{xie2020chexplain}, %\jk{be confused about what? how confused?},
as people may have very distinct thresholds in mind to determine a valid prediction by the probabilities (\textit{e.g.}, 90\% is trustful for some people but some other people want it to be over 95\% to trust). 
Instead, \system presents simplified labels following four ranges: Highly Likely (75\% - 100\%), Likely (50\% - 75\%), Unlikely (25\% - 50\%), and Highly Unlikely (0\% - 25\%). 
Along with the failure types, \system shows the grayscale saliency map generated by Grad-CAM \cite{selvaraju2017grad}, which represents the important region used for prediction which can thus highlight the point of interest. 
This is to help users comprehend the problematic parts in the photo, as well as to provide explainability of CNN models' decision~\cite{preece2018asking}.% \jk{why is providing explainability important to users?}
As in Figure~\ref{figure:system_diagnosis}, the `Show AI's Best Guess' is activated by default which makes the `Highly Likely' failure type visible solely. 
Upon preference, a user can also enable seeing all failure types, to help him make his own decision by checking and evaluating CNN classification models' performance on all failure types, if he wish to check all types' prediction results and compare the representative images of the failure to uploaded images.
%\jk{does seeing all failure type guarantee that the user 'evaluate' the model's performance??}.
\nk{No it does not guarantee that. If they are more alert on ai's performance when they are using this type of tool (AI-driven)}

%by clicking the `Show All Failure Types' button.

\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/3DPFIX_description.png}
    \caption{The bottom section of the interface has 3 tabs to investigate solutions for the selected failure type by the module in Fig. \ref{figure:system_diagnosis}. The first tab, `What's This Problem?' shows example photos about the common visual characteristics of a failure type, as well as an easy-understandable description on the right.}
    \Description{}
    \label{figure:system_description}
    %  \vspace{-2.0ex}
\end{figure*}


\subsubsection{User benefit 2: Learning Types of Failure by Auto-diagnosis.}
\jk{where did the learning of 'terminology' go from this process?}
Upon clicking each failure type predicted, \system provides the detailed description about it, such as what it is called among other users of 3D printing, what may cause it, which appearances that failure type might have
%\jk{add what the detailed description tells users} 
under the (\textit{`What's this problem?'}) tab, as shown in Figure~\ref{figure:system_description}.
This tab also discloses several representative images that present different visual features that are extracted from our image dataset (See Figure~\ref{visual_features}).
These images assist users to understand common visual characteristics that the failure type can have, facilitating learning about print failures by seeing the possible different appearances of them have been exhibited in various users' cases.
% to refer to other online resources %\jk{why does the user need to refer to other online resources?}.

%Also, the users can learn the various visual features of the failure by looking at related images from other users.
%We elaborate more on generating the grayscale saliency map later in Section~\ref{technitcal_implementation}.


\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/3DPFIX_solutions.png}
    \caption{}
    \Description{}
    \label{figure:system_solutions}
    %  \vspace{-2.0ex}
\end{figure*}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/3DPFIX_hoverover.png}
    \caption{}
    \Description{}
    \label{figure:system_hoverover}
    %  \vspace{-2.0ex}
\end{figure}

\subsubsection{User benefit 3: Learning Common \& Specific Solutions.}
Once the user got to know the details about the type of print failure, the terminology, visual characteristics, and what causes them, s/he can now move to the next step to learn about solutions.
\system provides two tabs for the curated solution-seeking which leads users to follow a reasonable flow \jk{why is it reasonable?} of troubleshooting. 
The user
%\jk{match the subject (number)} 
can begin with exploring common solutions which is likely to solve the most of cases under the `See Common Solutions' tab as shown in Figure~\ref{figure:system_solutions}a).
For two tabs for solutions% \jk{what is both here?}
, users can have noticeable situations or settings 
%\jk{what does 'specific' situation mean here?} or settings
, which we will refer to `clue'.
For examples, the user might 
The clue, possible situations (\textit{e.g.}, popping noise while printing, bed is wobbling) or settings (\textit{e.g.}, printing temperature was lower than 180 degree when using PLA, installing new firmware) that the user might have,
%\jk{add what it means: e.g., characteristics that might eventually cause the issues} 
may lead users to the specific solution set.
For example, if a user has a under-extrusion issue with PLA at lower than 180 degree for nozzle temperature as her setting, a low temperature of the print nozzle is likely to be a cause not being able to completely melt and fuse PLA \cite{printing_temperature}. 
Thus, the first-class suggestion could become increasing nozzle temperature around 210 degree that tend to work across many machines.
If users can spot any from the list of \textit{clues}, users can filter the relevant solutions quickly by navigating through each options.
The `Common Solution Did Not Work?' tab in Figure~\ref{figure:system_solutions}b) present solutions for more specific cases.
This can be helpful for users who were not able to resolve their issues by trying the most common solutions suggested in the previous tab.
Users can use the filter and sort solutions by difficulty level in decision making. For more intuitive design, the color scheme of the solution cards reflects the difficulty level.
The solution card is presented with the title and a short description to convey the information quickly and effectively at a glance. 
If the user% \jk{match the number} 
requires more detail such as how to deal with Cura (one of the most well-used slicing software) to increase the nozzle temperature, they can click `View Detail' or `View Video' in the solution cards that will direct them to the relevant online web tutorial document or video for more in depth information, if needed.
As Figure~\ref{figure:system_hoverover} shows, \system further aids newcomers learn technical terms used in the text describing solutions by hovering over them (Design Consideration \#n. ), enabling novices quickly learn from it without any further research outside of \system.



\subsubsection{Implementation.} \label{technitcal_implementation}
The web-based user interface enables users to upload images of their problematic 3D printed models.
%, utilizing all resources and image dataset available back-end without installing the software locally. 
The back-end framework is built on Flask \cite{} a lightweight web application framework written in Python. 
Having a Python-based back end enables real-time model classification and visual explanation generation using our pre-trained deep learning models, post-hoc explanation techniques (Grad-CAM), and data visualization libraries used (PyTorch, Matplotlib, OpenCV). 
The front end is written in basic HTML, CSS, JavaScript, and additional libraries (D3, jQuery) for dynamic elements.
The visual explanation is generated by Grad-CAM \cite{selvaraju2017grad} PyTorch library, which is a popular post-hoc technique that computes the gradient saliency maps~\cite{simonyan2013deep}
to visualize the model prediction by highlighting ‘important’ pixels (i.e., change in intensities of these pixels have the most impact on the prediction score).
%\nk{Do you need the GitHub for Grad-CAM lib?}
%For each failure type, the library generates a matrix consisting of attention scores (normalized to a 0-to-1 range) to which the trained model for predicting a failure type pays attention. 
%For a clear visualization of model-focused areas on the photos, 
All maps are transformed into grayscale by applying a sigmoid (slope = 4) to the model-generated attention scores pixel-by-pixel. 
This allows segmenting the attention areas (transparent mapping) from non-attention areas (dark mapping). 
Users can assume that a model's judgment of a failure type was made by looking at the attention areas of this saliency map. 
%\jk{add what this means to users}. 
The brighter the mapping, the higher the attention of the model. Then, each saliency map is passed to the front end as a clickable tab for each prediction. 
By choosing one, the interface will show the corresponding introduction, clues, and solutions relevant to the selected failure type at the bottom for the user's further investigation.









%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{High-level User Workflow with Design Considerations}
We elaborate on the high-level user workflow with the design considerations that we clarified in the formative study in Section~\ref{design_considerations}. 3DPFIX has mainly two interfaces, the initial page to upload the photos and the main page for diagnosis and solution seeking. Reflecting the first design requirement (\textit{image-based automatic diagnosis of failure}) 3DPFIX asks users to upload the photos of the user prints to provide a deep learning-based diagnosis at the initial user interface. After uploading the photos, users can select the image to explore on the top of the main interface. For the selected image, the interface shows the cards that represent the most viable failures with high prediction probabilities. Along with the failure type, users can see the grayscale saliency map per each image that represents the attention of the deep learning model. If needed, users can see the saliency map to understand which part of the photo shows the visual characteristics of the failure. 
3DPFIX support three different tabs for the selected failure type. If users click each failure type card, 3DPFIX first shows the description of the failure that we got from the Simplify3D’s guide \cite{simplify3d} under the `What’s This Problem?' tab. Users can navigate two other tabs, for common solutions (`See Common Solutions') and more specific solutions (`Common Solution Did Not Work?'), to seek what to do to resolve the failure. Common solutions 

It is also possible that users’ failure is specific and cannot be easily solved by the common solutions. If they could not resolve the failure after trying common solutions, users then can click the third tab for specific solutions, which we extracted from the community posts that cover the possible cases in a very comprehensive way. If they spotted 

Since our prototype supports 5 failure types, 



%T.B.D. 
static images and texts in the online tutorial documents created by experts do not assist them to spot similarities to their problem to locate solutions. The popular online guides (\textit{e.g.}, \cite{simplify3d, reprap}) only provide a single representative image for each failure type, so that users must map the visual characteristics of their own printing failure to this limited visual aid by themselves to be able to successfully categorize their 3D printing problem and thus find the solution. 
\end{comment}
